A many-body characterization of the fundamental gap in monolayer CrI$_3$

The many-body fixed-node and fixed-phase spin-orbit Diffusion Monte Carlo (DMC) methods are applied to accurately predict the fundamental gap of monolayer CrI$_3$ - the first experimentally-realized 2D material with intrinsic magnetism. The fundamental gap obtained, 2.9(1)~eV, agrees well with the highest peak in optical spectroscopy measurements and a previous $GW$ result. We numerically show that as expected in DMC the same value of the fundamental gap is obtained in the thermodynamic limit using both neutral promotions and the standard quasiparticle definition of the gap based on the ionization potential and electron affinity. Additional analysis of the differences between density matrices formed in different bases using configuration interaction calculations explains why a single-reference trial wave function can produce an accurate excitation. We find that accounting for electron correlation is more crucial than accounting for spin-orbit effects in determining the fundamental gap. These results highlight how DMC can be used to benchmark 2D material physics and emphasize the importance of using beyond-DFT methods for studying 2D materials.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> xx.tex <==


